VisionArena: 230K Real World User-VLM Conversations with Preference Labels

With the growing adoption and capabilities of vision-language models (VLMs) comes the need for benchmarks that capture authentic user-VLM interactions. In response, we create VisionArena, a dataset of 230K real-world conversations between users and VLMs. Collected from Chatbot Arena - an open-source platform where users interact with VLMs and submit preference votes - VisionArena spans 73K unique users, 45 VLMs, and 138 languages. Our dataset contains three subsets: VisionArena-Chat, 200k single and multi-turn conversations between a user and a VLM; VisionArena-Battle, 30K conversations comparing two anonymous VLMs with user preference votes; and VisionArena-Bench, an automatic benchmark of 500 diverse user prompts that efficiently approximate the live Chatbot Arena model rankings. Additionally, we highlight the types of question asked by users, the influence of response style on preference, and areas where models often fail. We find open-ended tasks like captioning and humor are highly style-dependent, and current VLMs struggle with spatial reasoning and planning tasks. Lastly, we show finetuning the same base model on VisionArena-Chat outperforms Llava-Instruct-158K, with a 17-point gain on MMMU and a 46-point gain on the WildVision benchmark. Dataset at https://huggingface.co/lmarena-ai

==> sec/0_abstract.tex <==
\begin{abstract}
\joey{Abstract is too long!! }
The growing adoption and capabilities of vision-language models (VLMs) demand benchmarks that reflect real-world user interactions. 
We introduce \dataset{}, the largest existing dataset of crowdsourced 
real-world conversations 
between users and VLMs. While most visual question-answering datasets focus on close-ended problems or synthetic scenarios, \dataset{} contains a wide variety of closed and open ended problems across 230K conversations, 73K unique users, 138 languages, and 45 VLMs. \dataset{} consists of \textbf{VisionArena-Chat}, a set of 200k single-turn and multi-turn chat logs with a VLM,  \textbf{VisionArena-Battle}, a set of 30K conversations between a user and 2 anonymous VLMs with preference votes, and \textbf{VisionArena-Bench}, an automatic benchmark consisting of 500 diverse user prompts which can be used to cheaply approximate model rankings.

We analyze these datasets and highlight the types of question asked by users, the influence of style on user preference, and areas where models often fall short. We find that more open-ended questions like captioning and humor are heavily influenced by style, which causes certain models like Reka Flash and InternVL which are tuned for style to perform significantly better on these categories compared to other categories.
We show that VisionArena-Chat and VisionArena-Battle can be used for post-training to align VLM's to human preferences through supervised fine-tuning. Compared to the popular instruction tuning dataset Llava-Instruct-158K, finetuning the same base model on \dataset{} results in a 17 point improvement on MMMU and a 46 point improvement on the WildVision human preference benchmark.
\joey{Wow!!! Keep this in the final abstract.}
Lastly, we show that running automatic VLM evaluation on VisionArena-Bench results in a model ranking which is largely consistent with major online preference benchmarks. We release both \dataset{} and our finetuned model to further VLM development. 
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}


Visual language models (VLMs)~\cite{openai2023gpt4,reid2024gemini,claude32024family,llama3modelcard} are being increasingly used in a wide range of real-world applications including image captioning and story telling, document understanding, web development, and embodied systems. 
While these models have made remarkable progress on a wide range of benchmarks~\cite{VQA,yue2024mmmumassivemultidisciplinemultimodal,balanced_binary_vqa,balanced_vqa_v2,gurari2018vizwiz,gurari2019vizwizpriv}, 
% remain largely focused on tasks with predefined ground truth answers. 
these visual question-answering benchmarks often contain close-ended questions, failing to capture the open-ended and complex nature of real-world applications and user interactions.


\begin{table*}[h]
\centering
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrrrrr}
\toprule
\multirow{2}{*}{Dataset} & \multirow{2}{*}{\# Convs} & \multirow{2}{*}{\# Models} &  \multirow{2}{*}{\# Users} & \multirow{2}{*}{\# Langs} & \% Unique Images & Avg. \# Turns & Avg. \# Tokens & Avg. \# Tokens & Human   \\
&  &  & &  & per Sample  &  & per Prompt & per Response & Preference\\
\midrule
\midrule
LMSYS-Chat-1M & 1,000,000 & 25 & 13,500 & 35 & - & 2.0 & 36.9 & 214.2 & No & \\
WildVision-Battle & 10,383 & 19 & - & 28 & 56.2 & 1.2 & 57.8 & 131.7 & Yes & \\
WildVision-Chat & 45,170 & 9 & - & 26 & 33.4 & 1.4 & 81.3 & 171.6 & No & \\
\midrule
\dataset{}-Battle & 30,000 & 17 & 14,031 & 90 & 76.4 & 1.3 & 90.2 & 393.6 & Yes & \\
\dataset{}-Chat & 200,000 & 45 & 72.933 & 138 & 62.1 & 1.5 & 184.1 & 634.3 & No & \\
\bottomrule
\end{tabular}%
}
\caption{\textbf{Dataset Comparison.} Compared to previous VLM preference benchmarks, \dataset{} contains 3x the amount of data, with more users, language, models, unique images, and conversation turns.}
\label{tab:dataset_comparrison}
\end{table*}

Understanding these real-world interactions across a variety of tasks is essential for developing models that align with human expectations and perform effectively.
% across diverse scenarios. 
To address this, previous works such as Chatbot Arena~\cite{chiang2024chatbot} and WildVision~\cite{lu2024wildvision,yujie2024wildvisionv2} crowdsource evaluation by hosting platforms where users can freely interact with pairs of VLMs and provide preference votes. 
Building off of these works, we introduce \textbf{\dataset{}}, a dataset of 230K real-world conversations between users and 38 VLMs in 135 languages. \dataset{} consists of:

\begin{itemize}
    \item \textbf{\dataset{}-Chat}: 200,000 single-turn and multi-turn chat logs between users and VLMs, covering a wide range of queries and responses.
    \item \textbf{\dataset{}-Battle}: 30,000 conversations where users interact with two anonymized VLMs, along with preference votes indicating which response they prefer.
    \item \textbf{\dataset{}-Bench}: An automatic benchmark consisting of 500 diverse user prompts that can be used to cheaply approximate model rankings via automatic benchmarking with VLM as a judge. 
\end{itemize}

We perform an analysis of the data and construct a set of popular question categories including captioning, OCR, humor, creative writing, entity recognition, and diagram understanding. We also explore the influence of stylistic properties of responses such as response length, markdown, and specificity on human preference. We find that more open-ended questions like captioning and humor are heavily influenced by style, which causes certain models like InternVL to have a disproportionately higher ranking in these categories. 
We provide this metadata with \dataset{} to enable further analysis. We also highlight common failure modes of VLMs and provide a small curated set of user prompts where top proprietary models fail.

Next, we demonstrate how \dataset{} can be used to improve VLMs through instruction fine-tuning. Compared to LLaVA-Instruct-158K~\cite{liu2023visualinstructiontuning}, by fine-tuning on data from VisionArena-Chat, models show a 17 point improvement in MMMU~\cite{yue2024mmmumassivemultidisciplinemultimodal} and a 46 point improvement on the human preference benchmark WV-Bench~\cite{lu2024wildvision}. In addition to \dataset{}, we also release this finetuned model. 
Lastly, we build on existing work in automatic benchmarking of VLMs to show that evaluating on the 500 prompts in VisionArena-Bench results in a model lineup that is consistent with the much larger online preference leaderboard Chatbot Arena. When compared with other automatic preference benchmarks like WildVision-Bench,  \dataset{}-Bench is far more predictive of the online Chatbot Arena VLM leaderboard performance, which contains over 100,000 user votes as of October 23rd, 2024. We believe that \dataset{} is a valuable resource to better understand how people are currently using VLMs and will be the foundation for future research in VLM development and evaluation. 

==> sec/analysis.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/tsne/topics_top5.pdf}
    \caption{\textbf{Comparison of top 5 topic clusters between WildVision-Chat and VisionArena-Chat.} Compared to WildVision, the most popular topics clusters in \dataset{} capture more real world tasks, specifically in STEM fields.}
    \label{fig:topics_5}
    \vspace{-1em}
\end{figure}


\section{Data Analysis}
\label{sec:analysis}

In the following section, we (1) compare user votes to expert annotators (2), analyze and categorize the distribution of user conversations (3), compute per category leaderboard (4), measure the impact of response style on human preference, and (5) provide examples of difficult questions. 

\subsection{Comparing with Experts and the VisionArena}
To inspect the quality of the human preference votes on our platform, we check their alignment with experts opinions. 
We sample 5 battles in English for each model pair and have 4 experts (PhD Students) label the battles based on their preference, creating an expert-labeled dataset of 516 responses.

We then compute BT scores using the expert labels and compare those scores with the BT scores computed directly on the VisionArena. 
We then compute the Pearson correlation coefficient~\cite{pearson} and the Spearman rank correlation coefficient~\cite{Spearman1904}. 
We obtain a Pearson correlation of 0.88
indicating a strong linear predictive relationship between the BT scores computed by experts and those obtained from the live VisionArena.
We obtain a Spearman rank correlation of 0.87
indicating high agreement in the ordering between the leaderboard rankings and the ranking obtained by our expert labelers on the small subset of data. 

Additionally, for a subset of 100 battles labeled by 3 experts, we observe an agreement of 0.72 (excluding ties) and 0.56 (including ties) between users and expert annotators, compared to 0.77 (excluding ties) and 0.59 (including ties) among expert annotators themselves, further demonstrating the reliability of user votes.

\subsection{What types of questions do people ask?}

We perform topic modeling analysis on the VisionArena-Chat prompts. Following the BERTopic framework, We randomly sample 50K English conversations and embed the documents using CLIP-ViT-B-32, perform DBSCAN clustering, and use GPT-4o to summarize each cluster \cite{grootendorst2022bertopic}. We plot our top 5 clusters in \autoref{fig:topics_5} (the top 20 clusters can be found in the supplement). We find that many people use VLMs to solve math and code problems, identify paintings and geographical locations, perform data analysis on tables and diagrams, explain humorous images, and create stories based on images. Notably, VisionArena-Chat contains important use cases not seen in WildVision-Chat including coding and web UI design problems, handwritten text extraction, and diagram analysis. Manually inspecting the clusters, we also see that WildVision-Chat's clusters are often very specific to a certain task (e.g. "Detailed Cartoon Dog Description", "Rice Leaf Disease Identification"), while VisionArena-Chat's cluster descriptions are broader which indicates the diversity of our data. Surprisingly, the majority of our questions require OCR, and we receive a large number of homework problems and diagram understanding questions. In the following section, we construct categories for each of these major use cases. 

\subsection{Prompt Categories}

\begin{figure}[h]
    \centering
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \small
        \begin{tabularx}{\textwidth}{lX}
            \toprule
            \textbf{Category} & \textbf{Description} \\
            \midrule
            \textit{Multi-Turn} & Conversations with multiple turns. \\
            \textit{Exclude Ties} & Battles which do not end in a tie. \\
            \textit{Exclude Refusal} & Neither model refuses to answer. \\
            \midrule
            \textit{Captioning} & \textit{Only} asks for a description of the image. \\
            \textit{OCR} & Requires reading text within the image. \\
            \textit{Coding} & Contains a code block in either the user inputs or model outputs. \\
            \textit{Entity Recognition} & Asks to identify objects, places, or people in the image. \\
            \textit{Homework} & Requires answering a problem which likely comes from a homework or exam. \\
            \textit{Humor} & Asks to explain the humor within the image or ask for a humorous composition. \\
            \textit{Diagram} & Contains images with a diagram (e.g., flowchart, circuit, graph). \\
            \textit{Creative Writing} & Asks for a creative composition such as a story or a script. \\
            \bottomrule
        \end{tabularx}
        \vspace{-1em}
        \caption{Descriptions of \dataset{} categories.}
        \vspace{3em}
        \label{tab:dataset_categories}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/category_proportion_plot.pdf}
        \vspace{-3em}
        \caption{\textbf{Category Distribution.} Excluding preset examples. We see that direct chat data contains a higher proportion of coding, homework, and diagram questions while battle data contains more captioning, humor, and creative writing questions.}
        \label{fig:category_counts}
        % \vspace{-1em}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \vspace{2em}
        \includegraphics[width=\linewidth, trim=0 0 0 0, clip]{figs/style_coeffs.pdf}
        \caption{\textbf{Impact of confounding variables on user preferences, measured by $\hat{\gamma}$ in the enhanced Bradley-Terry Model.} Length is by far the most influential stylistic factor, with higher influence on preference for more open ended questions like humor, creative writing, and captioning.}
        \label{fig:control_coefs}
        \vspace{-2em}
    \end{minipage}
\end{figure}

% \begin{table}[h]
%     \centering
%     \small
%     \begin{tabularx}{0.48\textwidth}{lX}
%         \toprule
%         \textbf{Category} & \textbf{Description} \\
%         \midrule
%         \textit{Multi-Turn} & Conversations with multiple turns. \\
%         \textit{Exclude Ties} & Battles which do not end in a tie. \\
%         \textit{Exclude Refusal} & Battles where neither model refuses to answer. \\
%         \midrule
%         \textit{Captioning} & \textit{Only} asks for a description of the image. \\
%         \textit{OCR} & Requires reading text within the image. \\
%         \textit{Coding} & Contains a code block in either the user inputs or model outputs. \\
%         \textit{Entity Recognition} & Asks to identify objects, places, or people in the image. \\
%         \textit{Homework} & Requires answering a problem which likely comes from a homework or exam. \\
%         \textit{Humor} & Asks to explain the humor within the image or ask for a humorous composition. \\
%         \textit{Diagram} & Contains images with a diagram (e.g., flowchart, circuit, graph). \\
%         \textit{Creative Writing} & Asks for a creative composition such as a story or a script. \\
%         \bottomrule
%     \end{tabularx}
%     \caption{Descriptions of \dataset{} categories.}
%     \label{tab:dataset_categories}
% \end{table}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{figs/category_proportion_plot.pdf}
%     \vspace{-2em}
%     \caption{\textbf{Category Distribution.} Excluding preset examples. We see that direct chat data contains a higher proportion of coding, homework, and diagram questions while battle data contains more captioning, humor, and creative writing questions.}
%     \label{fig:category_counts}
% \end{figure}x

\begin{figure*}[h]
    \includegraphics[width=\linewidth]{figs/category_final_ranking-30k-no-sc.pdf}
    \label{fig:category_leaderboard}
\vspace{-2em}
\caption{\textbf{\dataset{} Battle Results across question categories and languages.} Cells with * contain fewer than 100 votes. Some models achieve a much higher performance in certain categories, such as InternVL2 on captioning and Chinese, Reka Core on entity recognition, and Llava 1.6 on Humor. We also see models with a sharp drop in ranking on certain categories such as Reka Flash on multi-turn and diagrams, and Gemini 1.5 Flash/Pro on Chinese.}
\vspace{-1em}
\label{fig:category_battle_results}
\end{figure*}


Based on the clustering analysis and manual inspection, we manually define 8 non-disjoint categories that reflect the vast majority of prompts and test different capabilities of the VLM.
We use Gemini 1.5 Flash to classify each prompt, using both the image and text, into a set of predefined categories listed in \autoref{tab:dataset_categories}.
Section~\ref{sec:category_supp} contains detailed descriptions of each category, the prompts used to implement the categorization with 1.5 Flash, and the correlation between 1.5 Flash category labels and those of SOTA models.

\begin{figure*}
    \begin{subfigure}{1\textwidth}
    \includegraphics[width=\linewidth, trim=0 80 0 30, clip]{figs/cat_and_lang.pdf}
    \label{fig:battle_counts}
\end{subfigure}
\vspace{-2em}
\caption{\textbf{\dataset{} Change in rankings when style control is applied.} Cells with * contain battles with fewer than 100 votes. InternVL, Reka Flash, and Llava 1.6 see a ranking drop across the majority of categories, while Claude 3 Haiku and MiniCPM see an increase across most categories. The model lineup changes the most for the captioning, humor, and Vietnamese categories.}
\vspace{-1em}
\label{fig:style_control}
\end{figure*}

% \begin{itemize}
% \item\textit{Multi-Turn:} Conversations with multiple turns.

% \item\textit{Exclude Ties:} Battles which do not end in a tie.

% \item\textit{Exclude Refusal:} Conversations where neither model refuses to answer. 

% \item\textit{Captioning:} Conversations which \textit{only} ask for an unrestricted description of the image. Prompts which ask for a directed explanation (e.g. describe what is funny about this image) are not considered captioning questions. 

% \item\textit{OCR:} Conversations which require reading text within the image.

% \item\textit{Coding:} Conversations which contain a code block in either the user inputs or model outputs. 

% \item\textit{Entity Recognition:} Conversations which ask to identify objects, places, or people in the image. 

% \item\textit{Homework:} Conversations which ask to answer a problem which likely comes from a problem set or exam. 

% \item\textit{Humor:} Conversations which ask to explain the humor within the image or ask for a humorous composition (e.g. write a funny caption for this image)

% \item\textit{Diagram:} Conversations which contain images with a diagram (e.g. flowchart, circuit, graph). 

% \item\textit{Creative Writing:} Conversations which ask for some creative composition such as a story, a joke, or a script. 
% \end{itemize}


\autoref{fig:category_counts} shows the distribution of category counts for both battles and direct chat conversations. We observe that direct chat conversations contain more homework and diagram understanding problems while battles contain more humor, captioning, and creative writing problems. We speculate this is because users in direct chat mode are more interested in using proprietary VLMs at no cost to assist them with their daily tasks. 

Model rankings and Arena Scores for select categories and languages are shown in \autoref{fig:category_battle_results} (full table and arena scores can be found in the supplemental). We find several interesting insights such as: 

\begin{itemize}
    \item Gemini 1.5 Pro Exp~\cite{reid2024gemini}, InternVL~\cite{chen2024far,chen2023internvl} and Reka Flash~\cite{rekateam2024rekacoreflashedge} achieve a worse ranking for categories with require OCR like coding, homework, and diagrams. 
    \item InternVL has a large improvement in ranking for the captioning category. In the following section, we show that this is largely due to stylistic choices such as formatting. 
    \item Claude Opus, Sonnet, and Haiku~\cite{claude32024family} see an increase in ratings for multi-turn conversations.
    \item The Gemini class of models drops in performance on non-english conversations.
\end{itemize}


\subsection{Controlling stylistic biases in evaluations}
\label{sec:style_analysis}

The Vision Arena captures signals from users of various backgrounds and preferences to construct its leaderboard. However, recent literature has pointed out potential confounding variables in model evaluation such as the length of the response or stylistic formatting \cite{chiang2024chatbot, dunlap_vibecheck}. Others have also mentioned various axes in which annotators may disagree including task underspecification, response style, refusals, and annotation errors \cite{zhang2024divergingpreferencesannotatorsdisagree}. Thus, we explore the effect of these stylistic features on the VisionArena user preference. 

We follow recent work that extends the BT model to include style features \cite{li2024crowdsourceddatahighqualitybenchmarks}. Given a set of style features (e.g. response length, number of markdown headers), we add a style vector to the BT model $\vec{Z}$ where=
    $Z_i \in \mathbb{R}^S$ is a vector of $S$ style features.
the enhanced BT model has the style coefficients $\gamma \in \mathbb{R}^{S}$:
\begin{align*}
    \hat{\beta}, \hat{\gamma} = \arg \min_{\beta \in \mathbb{R}^M, \gamma \in \mathbb{R}^S} \frac{1}{n}\sum\limits_{i=1}^n \text{CE}(\sigma(X_i^\top \beta + Z_i^\top \gamma), Y_i)
\end{align*}
 For each style feature $Z_i$, we compute the normalized feature difference between the model responses. 
 The resulting $\hat{\beta}$ represents model strengths adjusted for style effects, while $\hat{\gamma}$ quantifies the influence of style on user preferences.
 
To control for these stylistic factors, we modify how \dataset{} computes the model scores by accounting for the stylistic differences between two answers (response length, number of markdown headers, etc) as additional features to the existing BT model.

\noindent\textbf{Controlling for length and markdown.} Applying style control, we see the captioning category is heavily affected by style, with \autoref{fig:style_control} showing a large difference in model rankings. We suspect this is because VLMs are heavily optimized for captioning and can usually correctly identify the main subjects and context of the image. This is supported in \autoref{tab:bothbad_counts}, which shows captioning questions have the smallest proportion of `both bad' votes. In cases where both models provide a reasonable description of the image, the user may rely on stylistic features to determine preference.

Furthermore, we also find that models like InternVL and Reka Flash Preview see a large decrease in rankings when style control is applied. We see that these models have an unusually high token output count when compared to models of a similar class (see supplemental). This indicates that some models may be `preference hacking' by optimizing for long or well formatted outputs. 

\begin{table}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{cccccccc}
    \toprule
     Caption & Homework & OCR & Coding & Humor & \shortstack{Entity \\ Recog.} & \shortstack{Creative \\ Writing} & Diagram \\
    \midrule
    11.33 & 31.12 & 20.62 & 29.4 & 18.47 & 22.25 & 14.21 & 26.06 \\
    \bottomrule
    \end{tabular}%
    }
    \vspace{-0.5em}
    \caption{\textbf{Percentage of `tie (bothbad)' per category.} Captioning, creative writing, and humor categories have low percentages of bothbad responses compared to coding and homework problems.}
    \label{tab:bothbad_counts}
    \vspace{-1em}
\end{table}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth, trim=0 0 0 0, clip]{figs/style_coeffs.pdf}
%     \caption{\textbf{Impact of confounding variables on user preferences, measured by $\hat{\gamma}$ in the enhanced Bradley-Terry Model.} Length is by far the most influential stylistic factor, with higher influence on preference for more open ended questions like humor, creative writing, and captioning.}
%     \label{fig:control_coefs}
% \end{figure}

\noindent\textbf{Controlling for specificity.} We further extend the Bradley-Terry model to include the effect of response specificity.
% We define the complexity of a response as the number of named entities in the response. 
To measure the specificity of a response, we use a NER model \cite{NOTHMAN2013151} to tag each response and use the number of named entities as our specificity score. In \autoref{fig:control_coefs}, we see that users prefer high specificity for tasks like entity recognition and diagram understanding while placing less emphasis on specificity for tasks like captioning and homework.
% In Figure \ref{fig:control_coefs}, We show that users prefer high specificity for tasks like entity recognition and diagram understanding while placing less importance on specificity for tasks like captioning and homework.
% We utilize the multilingual named entity tagger xx\_ent\_wiki\_sm which was trained on multilingual Wikipedia documents \cite{NOTHMAN2013151}. 
% To measure a hallucination in a response, we prompt a VLM (gemini-1.5-flash) to annotate the image and model response to detect whether the response includes objects, scenes, or details not present in the image (see section \ref{prompt:hallucination} for the full system prompt). 
% To measure the subjectivity of the response, we prompt a VLM (e.g. gemini-1.5-flash) to annotate whether the response contains extensive interpretative detail (classification prompt located in Section \ref{prompt:subjectivity}).

% \begin{table*}[h]
%     \centering
%     \resizebox{0.9\textwidth}{!}{%
%     \begin{tabular}{ccccccccc}
%     \toprule
%      & Overall & Homework & OCR & Humor & Entity Recognition & Creative Writing & Diagram & Captioning \\
%      \midrule
%      Length            & 0.257  & 0.201  & 0.248  & 0.284  & 0.168  & 0.329  & 0.199  & 0.444 \\
%     Markdown Header   & -0.008 & -0.002 & -0.008 & -0.008 & -0.012 & -0.004 & -0.038 & -0.039 \\
%     Markdown List     & -0.021 & -0.025 & -0.019 & -0.077 & -0.066 & -0.028 & -0.007 & -0.035 \\
%     Markdown Bold     & 0.049  & 0.035  & 0.053  & 0.026  & 0.164  & -0.048 & 0.069  & 0.066 \\
%     Hallucination     & -0.070 & -0.039 & -0.057 & -0.030 & -0.125 & -0.040 & -0.033 & -0.210 \\
%     Entity Counts     & 0.129  & 0.084  & 0.139  & 0.122  & 0.247  & 0.120  & 0.150  & 0.088 \\
%     Subjective Interpretation      & 0.042  & -0.047 & 0.005  & 0.072  & 0.007  & 0.121  & 0.007  & 0.051 \\
%     \bottomrule
%     \end{tabular}%
%     }
%     \vspace{-0.5em}
%     \caption{The influence of confounding variables in a user's preference measured by $\hat{\gamma}$, the coefficient in the enhanced Bradley-Terry Model \lisa{\textbf{Joseph Edgar Gonzalez please tell us how to graph this}}}
%     \label{tab:control_coefs}
% \end{table*}

\subsection{Failure Cases}

\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim=0 0 0 0, clip]{figs/cat_example.pdf}
        \caption{\textbf{Failure case 1.}}
        \label{fig:cat_example}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim=0 0 0 0, clip]{figs/train_line_example.pdf}
        \caption{\textbf{Failure case 2.}}
        \label{fig:train_line_example}
    \end{subfigure}
    \caption{\textbf{VLM failure modes.} Outputs are truncated, full outputs in the supplemental section. Even the top proprietary models fail at answer questions which require advanced visual reasoning.} 
    \vspace{-1em}
    \label{fig:failures}
\end{figure*}

We use \dataset{} to analyze examples which are particularly challenging for current VLMs.
% While VLMs have served as an incredible resource for many users on our platform, there are many simple cases where they fail. We demonstrate how the dataset can be used to find cases where models fail and where humans would succeed.
We first filter VisionArena-Chat for prompts where the user voted that both models are bad, and collect a pool of 10 images which most or all of the current VLMs fail. The full set can be found in the supplemental section.
% We divide failure cases into three categories: hard OCR, counting, and reasoning. Lastly, we provide examples of hard examples on which most or all of the current VLM's fail, with additional examples in Section~\ref{sec:failures_supp}.
\autoref{fig:cat_example} shows two examples of user questions that require advanced visual reasoning. This example requires the model to (1) understand that the two cats in the image are the same (2) the pattern on the cats back gives the illusion of another cat (3) this illusion of a smaller cat in a cat can be related to the fact that the square root of a number is a smaller demonimation of that number. \autoref{fig:train_line_example} is an example of fine-grained spatial understanding, as the model must locate both locations and reason over the many intersecting lines in the image. Analysis of other failure cases in the supplemental section indicates that current VLMs still struggle on visual grounding tasks like reading distorted images, spatial understand and counting, as well as more complex reasoning tasks. 



==> sec/dataset.tex <==

\definecolor{gray}{gray}{0.8}
\definecolor{gold}{rgb}{0.85, 0.65, 0.13}
\definecolor{darkbrown}{rgb}{0.6, 0.4, 0.2}
\definecolor{blackish}{rgb}{0.2, 0.2, 0.2}



\section{Dataset and Platform}
\label{sec:dataset}

\subsection{Interface}

VisionArena-Chat and VisionArena-Battle were collected from our open-source platform for evaluating large language models by human preference. 
On our platform, users are able to directly chat with specific models (direct chat) or chat with pairs of anonymous models side-by-side (battle mode). In battle mode, users can provide direct feedback on which responses they preferred, which is used to build a leaderboard. We refer to these anonymous side-by-side chats as `battles'. An example of our interface can be found in the supplemental. Unlike previous VLM crowdsourcing platforms, we integrate LLMs and VLMs into one unified chat interface with a simple routing mechanism. In side-by-side chat, if a user uploads an image in the first turn of their conversation, we automatically select from two available VLMs; otherwise we sample from the available LLMs. We then collect the votes from the image conversations to compute the VLM leaderboard. We believe this encourages users who may have initially been interested in interacting with LLMs to interact with VLMs as well. In \autoref{sec:analysis}, we show that our conversations do have important distributional differences with WildVision. 

Before using our service, users must accept terms of use, giving us their consent to store and release the conversation data. The platform is free to use for all users, and there is no registration process. We are supported by sponsorships with inference providers. \dataset{} is a subset of conversations collected from February 2024 to September 2024. Given the language and question distribution of our collected conversations, the majority of our users are likely located in North America, Europe, and East Asia and work in STEM related fields. 

To encourage user interaction, we provide a `random image' button, which samples from a preset bank of images from 5 datasets: NewYorker~\cite{newyorkernextmldataset}, ChartVQA~\cite{masry-etal-2022-chartqa}, DocVQA~\cite{mathew2020docvqa}, TextVQA~\cite{singh2019towards}, and WikiArt~\cite{wikiart}. We exclude these in VisionArena-Battle as we aim to capture the natural distribution of user inputs when computing leaderboard rankings. We release conversations with preset images in VisionArena-Chat, which make up around 15\% of conversations. 

\noindent\textbf{Moderation.} We apply several moderation steps before sending the prompt to the model provider and perform data cleaning procedures before releasing this data to the public.
Before the user receives the response from the model, we perform (not safe for work) NSFW image detection and (child sexual abuse material) CSAM~\cite{PhotoDNA} image detection and then tag and terminate conversations that contain inappropriate content.
For battles, we also perform OpenAI text moderation~\cite{OpenAITextModeration} on user text prompts and discard any responses which contain a violation. For direct chats, we only perform OpenAI text moderation on proprietary models to follow their usage policies. We do not perform text moderation on prompts for open-source models, which opens this data for future analysis. 

Finally, as part of our data release process we use Google’s Vision API~\cite{googlevision} to remove personally identifiable information (PII) from both images and text, removing any content containing human faces or identifiable details.

\subsection{From Preference to Leaderboard Ranking}
\label{sec:leaderboard_calculation}

Using preference votes from pairwise battles in anonymous side-by-side chat, we apply a Bradley-Terry (BT) model~\cite{BradleyTerry1952} to estimate the relative strengths of models through logistic regression. The model’s coefficients serve as \textit{arena scores}, which determine the leaderboard rankings.

Let $n$ denote the number of pairwise comparisons (battles) and $M$ the number of models. 
For each battle $i \in [n]$, we define:
\begin{itemize}
    \item $X_i \in \mathbb{R}^M$: $X_{i,m} = 1$ if model $m$ is presented first to the judge, $X_{i,m} = -1$ if presented last, and 0 otherwise.
    \item  $Y_i \in {0,1}$: The outcome, where 1 indicates the first model won.
\end{itemize}



The BT model estimates model strengths $\beta \in \mathbb{R}^M$ through logistic regression:
\begin{equation}
\hat{\beta} = \arg \min_{\beta \in \mathbb{R}^M} \frac{1}{n}\sum\limits_{i=1}^n \text{CE}(\sigma(X_i^\top \beta), Y_i)
\end{equation}
where $\text{CE}$ represents the cross-entropy loss and $\sigma$ is the sigmoid function. 
The BT coefficients $\hat{\beta}$ are the ratings associated with each of the VLMs in the arena.
These BT ratings are used to create the ordered ranking of models on the leaderboard. 
We bootstrap the BT rating estimate 100 times to construct a confidence interval for each rating.



==> sec/finetuning.tex <==
% \section{Applications} 
% \label{sec:applications}

% \begin{table}[ht]
% \centering
% \begin{tabular}{lccc}
% \tiny
% \toprule
% \textbf{Benchmark} & \textbf{WV-Bench} &  \textbf{ArenaVQA} & \textbf{Arena-Hard-VQA} \\
% \midrule
% Confidence Agreement & 89.1\% & 66.7\% & 84.8\%  \\
% Separability         & 87.4\% & 83.68\% & 82.11\%  \\
% Spearman Correlation & 94.1\% & 77.0\% & 95.2\%  \\
% \bottomrule
% \end{tabular}
% \caption{Table comparing various benchmarks on different evaluation metrics. \textbf{\textcolor{red}{TODO: FILL THIS OUT}}}
% \end{table}

\section{Instruction tuning vision-language models}


\begin{table}[h]
\small
\centering
\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{Samples} & \textbf{MMMU $^5$} & \textbf{WV-Bench} \\
\midrule
Llama3.2-11B-V & - & 41.7 & - \\
\textcolor{darkgray}{Llama3.2-11B-V-Instruct} & \textcolor{darkgray}{3M+} & \textcolor{darkgray}{\textbf{50.7}} & \textcolor{darkgray}{47.2} \\
Llama-3.2-Llava-Instruct & 100K & 27.9 & 10.4 \\
Llama-3.2-VisionArena & 100K & 43.0 & \textbf{56.9} \\
\bottomrule
\end{tabular}%
}
\caption{\textbf{Performance comparison across different models.}  Scores for Llama-3.2-11B-Vision and Llama-3.2-11B-Vision-Instruct are author-reported. Finetuning with 100k samples from \dataset{} achieves an MMMU score 15 points higher than finetuning on Llava-Instruct data and a WV-Bench score 9 points higher than Llama-3.2-11B-Vision-Instruct. Despite being fine-tuned on 30x less data, Arena-11B performs comparably to Llama-3.2-11B-Vision-Instruct in chat tasks.}
\label{table:finetune}
\end{table}


Effective instruction fine-tuning for vision-language models depends on the diversity of instructions, the difficulty of prompts, and the quality of responses. This section demonstrates the potential of \dataset{} for training high-performance instruction-following models.

We curate a high quality instruction-tuning dataset by sampling from the conversations with the highest-performing VLMs. We choose 100,000 conversations from VisionArena-Chat from the top models. This led to a dataset with conversations from 16 different models\footnotemark[2] including proprietary models such as GPT-4o~\cite{openai2023gpt4}, Gemini-1.5-Pro~\cite{reid2024gemini},  and Claude-3.5-Sonnet~\cite{claude32024family} as well as open-source models such as Qwen2-VL-72B~\cite{Qwen-VL, wang2024qwen2vlenhancingvisionlanguagemodels} and Llama-3.2-90B-Vision-Instruct~\cite{llama3modelcard}. We compare the effectiveness of this dataset for finetuning to a 100K subset of Llava-Instruct-158K~\cite{liu2023visualinstructiontuning}, a popular VLM instruction following dataset. 

We use Llama-3.2-11B-Vision and freeze the vision encoder while fine-tuning the multimodal projector and language model. We finetune for 3 epochs on the data for both our 100k dataset and the 100k Llava-Instruct dataset. In \autoref{table:finetune}, we label the model finetuned on our \dataset{} data Llama-3.2-VisionArena and the model trained using Llava-Instruct-158K Llama-3.2-Llava-Instruct.

The evaluation results are shown in \autoref{table:finetune}. Llama-3.2-VisionArena achieves the highest WV-Bench score at 56.9 and increases the MMMU baseline by 1.3 points compared to the base model. This demonstrates the effectiveness of our fine-tuning data for both downstream chat tasks and overall performance.

\footnotetext[1]{gemini-1.5-pro-exp-0827, gemini-1.5-flash-exp-0827\cite{reid2024gemini}, gpt-4o-2024-05-13, gemini-1.5-flash-8b-exp-0827, internvl2-26b \cite{chen2024far}, claude-3.5-sonnet-20240620 \cite{claude32024family}, gpt-4-turbo-2024-04-09 \cite{openai2023gpt4}, claude-3-sonnet-20240229, llama-3.2-11b-vision-instruct \cite{llama3modelcard}, gemini-1.5-pro-001, internvl2-4b, gpt-4o-mini-2024-07-18, claude-3-opus-20240229, gemini-1.5-flash-001, reka-core-20240501 \cite{rekateam2024rekacoreflashedge}, claude-3-haiku-20240307}

\footnotetext[2]{gpt-4o-mini-2024-07-18, gpt-4-turbo-2024-04-09, gemini-1.5-pro-api-0514, claude-3-5-sonnet-20240620, gemini-1.5-pro-exp-0827, gpt-4o-2024-05-13, gemini-1.5-pro-exp-0801, gemini-1.5-flash-api-0514, claude-3-opus-20240229, gemini-1.5-flash-exp-0827, gemini-1.5-flash-8b-exp-0827, llama-3.2-vision-90b-instruct, qwen2-vl-72b \cite{wang2024qwen2vlenhancingvisionlanguagemodmodels2betweenels}, gpt-4o-2024-08-06, chatgpt-4o-latest-20240903, chatgpt-4o-latest-20240808}


\section{VisionArena-Bench: An Automatic Offline Human-Preference Benchmark for VLMs}

\begin{table}[h]
\small
\centering
\begin{tabular}{lcc}
\toprule
\textbf{} & \textbf{VisionArena-Bench} & \textbf{WV-Bench}  \\
\midrule
Confidence Agreement & \textbf{98.6\%} & 87.6\% \\
Spearman Correlation & \textbf{97.3\%} & 80.2\% \\
Kendall Tau Correlation & \textbf{89.7\%} & 69.2\% \\
\bottomrule
\end{tabular}
\caption{\textbf{Correlation of rankings with ChatbotArena's VLM leaderboard.} Performance comparison on 16 models\protect\footnotemark[1] between VisionArena-Bench to Chatbot Arena's VLM leaderboard based on confidence agreement, spearman correlation, and Kendall tau correlation. Result as of leaderboard on October 23, 2024.}
% \vspace{-1em}
\label{table:bench_results}
\end{table}

Lastly, we demonstrate \dataset{}'s ability to cheaply approximate model preference rankings with \dataset{}-Bench. Currently, online preference benchmarks like Chatbot Arena obtain a ranking for a new model by adding it to their platform and waiting days or weeks to collect enough votes for a stable ranking. For a single developer hoping to test a particular version of their model, obtaining these online model rankings is infeasible.
% Current benchmarks are static and based on ground-truth answers such as multiple choice, which does not reflect how users use VLMs on real-world tasks.While the Chatbot Arena VLM Leaderboard addresses these issues by recording human preference on battles, collecting sufficient votes may take days or weeks to estimate the model ranking properly. 
We develop a solution for those who need a quick and cheap evaluation of their models: VisionArena-Bench. VisionArena-Bench is a set of 500 diverse image and text prompts that accurately approximates the model ranking from the Chatbot Arena VLM Leaderboard. 

\noindent\textit{Offline benchmark curation.} To gather questions for this offline benchmark, we build on recent work in building benchmarks from crowd-sourced evaluations in LLM and adapt them to the context of VLM ~\cite{li2024crowdsourceddatahighqualitybenchmarks}. We first filter the data for single turn to prevent the user from correcting the model in its response on its second turn. We then filter out non-english conversations as we are personally unable to verify the quality of non-english prompts.

To sample diverse questions, we perform topic modeling using the library BERTopic with multimodal embeddings \cite{grootendorst2022bertopic}. We extract image embeddings and text embeddings using a CLIP model (e.g. CLIP-ViT-B-32) \cite{radford2021learningtransferablevisualmodels}. We then average the image and text embeddings so that each document corresponds to a single embedding. Then, we use UMAP to reduce the dimensions of the embedding and use hierarchical-based clustering (HDBSCAN) to generate topic clusters \cite{mcinnes2020umapuniformmanifoldapproximation, Malzer_2020}. We then uniformly sample from each topic cluster to generate the 500 prompts.

\noindent\textit{Automatic evaluation with VLM-as-a-judge.} To evaluate a model, we use the LLM-as-a-judge framework mentioned in \cite{li2024crowdsourceddatahighqualitybenchmarks} applied to VLMs. We first select a fixed anchor model (GPT-4-Turbo\cite{openai2023gpt4}) that will be used in the pairwise comparisons. To evaluate a given model $M$ on a user prompt $p$, we generate responses for both $M$ and the anchor model on $p$ and then utilize GPT-4o as a judge to provide a preference score between the ($M$, anchor) pair on a 5-point Likert scale. 1 indicates a strong preference for model A and 5 indicates a strong preference for model B. We then obtain this score for all models across all prompts in VisionArena-Bench to obtain VLM-generated pairwise preference votes and use the same procedure as described in \autoref{sec:dataset} to produce final model scores.
% We evaluate a model on a given image and prompt using a pairwise comparison against a strong baseline model GPT-4-Turbo \cite{openai2023gpt4}. We then utilize GPT-4o to score each output by rating its preference between the pair on a 5-point Likert scale. 1 indicates a strong preference for model A and 5 indicates a strong preference for model B, which effectively penalizes the model for significant losses. 
In the supplemental, we provide the detailed judge prompt template. To avoid potential bias, we prompt the judge model to judge twice, swapping the response position between the two rounds. 

To evaluate the effectiveness of our benchmark to existing work~\cite{lu2024wildvision}, we leverage standard metrics such as Spearman correlation and Kendall Tau correlation which measure the agreement between two benchmarks' model rankings. We choose a shared set of 16 models and compare the offline benchmark rankings to the online Chatbot Arena. We show in \autoref{table:bench_results} that using our simple benchmark creation strategy, we can achieve a Spearman correlation of 97.3\% and Kendall Tau correlation of 89.7\%, which is higher than other VLM benchmarks like WildVision-Bench by 17.1\% and 20.5\%, respectively. In the supplemental, we also compare the results using the same baseline model as WildVision (e.g. Claude-3-Sonnet-20240229), showing that the spearman correlation to Chatbot Arena's VLM leaderboard (10/23/2024) remains the same. This demonstrates the potential of VisionArena-Bench as a cost-effective and scalable offline benchmark that closely mirrors human preferences captured in online evaluations, enabling researchers to efficiently assess and compare VLMs without the need for extensive user studies.

==> sec/related_arxiv.tex <==
\section{Related Works}
\label{sec:related}

\textbf{Crowdsourced Evaluations.} In the past few years, several platforms have emerged that aim to crowdsource evaluation for LLMs and VLMs by allowing users to provide preference votes. These platforms, such as Chatbot Arena~\cite{chiang2024chatbot}, allow anyone to freely engage in open-ended conversations with state-of-the-art commercial and open-source models. Users are able to directly chat with specific models or chat with pairs of anonymous models side-by-side. In the anonymous side-by-side mode, users can provide direct feedback on which responses they preferred, which is used to build a leaderboard. WildVision~\cite{lu2024wildvision} adopts a similar style to Chatbot Arena except that users interact with VLMs instead of LLMs. Our platform builds upon these works by creating a unified interface that allows users to chat with \textit{either} LLMs or VLMs. 

\textbf{Public Chat Datasets:} LMSYS-Chat-1M~\cite{zheng2023lmsyschat1m}, OpenAssistant~\cite{kopf2023openassistant}, and WildChat-1M~\cite{kopf2023openassistant, deng2024wildvisopensourcevisualizer} are all public datasets constructed by capturing users conversations with state-of-the-art LLMs. 
These datasets have been highly influential because they represent more natural human conversations and often contain reward feedback signals. 
However, because these datasets capture text-only conversations,
they do not provide insight into how users incorporate images into conversations and the behavior of VLMs. 
Building on the success of public chat datasets, there is a recent effort to extend the public chat datasets to the visual domain with WildVision, a dataset of 45k chat logs with 9 visual question answering models and 10.4K battle logs across 19 models. In contrast, our \dataset{} data set contains 200K chat logs and 30K battle logs across 40+ models, including all of the strong proprietary models and many open-source models, making it the largest and most complete VLM conversation dataset to date. See Table~\ref{tab:dataset_comparrison} for dataset comparison. 
% It is important to note that while Chatbot Arena does have a VLM leaderboard with over 100,000 votes, they have yet to release any data to the public.

\textbf{VLM Benchmarks:} 
Currently, VLM benchmarks are typically static datasets that have close-ended ground truth answers (either multiple-choice or predefined-string). Some popular examples of these benchmarks include MMMU \cite{yue2024mmmumassivemultidisciplinemultimodal}, DocVQA \cite{mathew2020docvqa}, MME \cite{fu2024mmecomprehensiveevaluationbenchmark}, and VQA 2.0 \cite{goyal2017makingvvqamatter}. To combat against static nature of datasets and minimize test-set contamination, live benchmarks are also available. For example, LiveXiv incorporates updated ArXiv manuscripts for VQA \cite{shabtay2024livexivmultimodallive}. To incorporate benchmarking on open-ended responses, there has been a trend towards using strong models (e.g. GPT-4o) for VLM-as-a-judge to approximate human preference. Some notable examples include WildVision-Bench \cite{lu2024wildvision} and Prometheus-Vision \cite{lee2024prometheusvisionvisionlanguagemodeljudge}. We similarly adopt the VLM-as-a-judge framework to create \dataset{}-Bench, curated from questions from VisionArena, allowing it to be crowdsourced, open, and live. We show that using \dataset{}-Bench, we achieve better correlation and agreement with the VLM leaderboard on Chatbot Arena, which itself has 100x more votes.
